Long-tail learning via logit adjustment

Real-world classification problems typically exhibit an imbalanced or long-tailed label distribution, wherein many labels are associated with only a few samples. This poses a challenge for generalisation on such labels, and also makes na\"ive learning biased towards dominant labels. In this paper, we present two simple modifications of standard softmax cross-entropy training to cope with these challenges. Our techniques revisit the classic idea of logit adjustment based on the label frequencies, either applied post-hoc to a trained model, or enforced in the loss during training. Such adjustment encourages a large relative margin between logits of rare versus dominant labels. These techniques unify and generalise several recent proposals in the literature, while possessing firmer statistical grounding and empirical performance.

==> conclusion.tex <==
In this paper, we present two 
simple modifications of standard softmax cross-entropy training 
to cope with the problem of learning with long-tail labels.
Our techniques involve \emph{logit adjustment} based on the label priors,
either applied post-hoc to a trained model,
or enforced in the loss during training.
Such adjustment encourages a high \emph{relative margin} between logits of rare versus dominant labels.
Our techniques unify and generalise several recent proposals in the literature,
while possessing stronger 
theoretical guarantees
and empirical performance.


==> margin_defn.tex <==
%
{\color{red} These are some comments regarding our discussion on the margin for multi-class classification problem and its implications on learning in the presence of class imbalance.}

Let's assume that the scorer takes the form $f = W\cdot \phi$, where $W \in \Real^{L \times d}$ the so called classification layer and $\phi \colon \XCal \to \Real^d$ is the feature map that maps each instance to a $d$-dimensional embedding. In this case, the decision function is defined as 
\begin{align}
\label{eq:dec_mc}
h \colon x \mapsto \argmax_{y \in \YCal} w_y\cdot \phi(x).
\end{align}
This leads to the natural definition of multi-class margin for an example $(x, y)$
\begin{align}
\label{eq:margin_mc}
\gamma(x, y) = w_y\cdot\phi(x) - \max_{y' \neq y} w_{y'}\cdot\phi(x).
\end{align}
It follows from \eqref{eq:dec_mc} and \eqref{eq:margin_mc} that the scorer $f$ misclassifies the example $(x, y)$, i.e.,
\begin{align}
\label{eq:margin_err}
h(x) \neq y \quad \iff \quad \gamma(x, y) < 0.
\end{align}

Now, let's look at the binary classification problem for a moment. There, scorer function takes the simple form $f_{\rm b} = w_{\rm b}\cdot\phi$, with $w_{b} \in \Real^d$ and the decision function simply becomes
\begin{align}
\label{eq:dec_bin}
h_{\rm b} = {\rm sign} \big(w_{\rm b}\cdot \phi(x)\big).
\end{align}
This setup can be reduced to the multiclass classification setup (cf.~\eqref{eq:dec_mc}) by defining $W_{\rm b} = [w_{\rm b}; -w_{\rm b}] \in \Real^{2 \times d}$, i.e., $w_{\rm b}$ and $-w_{\rm b}$ form the classifiers for $+1$ and $-1$ classes, respectively. In the binary case, the (functional) margin is defined as
\begin{align}
\label{eq:f_margin_bin}
\gamma_{\rm f, b}(x, y) = y w_{b}\cdot \phi(x) = {\color{red}\frac{1}{2}} \cdot \left( w_{y}\cdot \phi(x) - w_{y'\neq y}\cdot \phi(x)\right),
\end{align}
which again agrees with the margin definition for the multiclass classification in \eqref{eq:margin_mc} (up to a scaling of $1/2$ which is just a matter of scaling). Again, the misclassfication even is tied to (functional) margin as
\begin{align}
h_{\rm b}(x) \neq y  \quad \iff \quad \gamma_{\rm f, b}(x, y) < 0.
\end{align}
So far so good, both binary and multiclass classifications are consistent. Also, if we only care about the misclassification on the training data, the margins as defined in \eqref{eq:margin_mc} and \eqref{eq:f_margin_bin} are all we need.

Now comes the generalization part. In the binary case, we want an example $(x, y)$ to be as far as possible from its classifier. The distance of $(x, y)$ from its classifier is defined as `geometric' margin, which takes the form
\begin{align}
\gamma_{g, b} = \frac{|w_{\rm b}\cdot\phi(x)|}{\|w_{\rm b}\|_2}.
\end{align}
Assuming that, we are correctly classifying $(x, y)$ by ensuring $\gamma_{\rm f, b}(x, y) > 0$, we can further increase the geometric margin by minimizing the norm $\|w_{\rm b}\|_2$. This gives rise to hard-SVM as
\begin{equation}
\begin{aligned}
\label{eq:binary_svm}
\min_{w} \quad & \|w_{\rm b}\| + \|-w_{\rm b}\| = 2\|w_{\rm b}\|_2\\
\textrm{s.t.} \quad & \gamma_{\rm f, b}(x_i, y_i) = y_i w_{\rm b}\cdot \phi(x_i) > 0~~\forall i \in [n].\\
\end{aligned}
\end{equation}
%
{\color{red} Sadeep: Not sure if I follow this. Isn't the geometric margin in (7) is independent of $\|w_b\|$?. Also, in hard SVM, do we not usually have a constraint $\gamma_{\rm f, b}(x_i, y_i) \ge 1$ (not zero) to ensure that we cannot make $\|w_b\|$ arbitrarily small.}
{\color{blue} Ankit: Yes, you are right. We should have $\gamma_{\rm f, b}(x_i, y_i) \geq \beta > 0$, with $\beta = 1$ as the common choice. Now, for support vectors, $\gamma_{\rm f, b} = \beta$ and $\gamma_{\rm g, b} = \frac{\beta}{\|w_{\rm b}\|_2}$, which can be maximized by minimizing $\|w_{\rm b}\|_2$. WDYT?}
{\color{red} Sadeep: I completely agree that after the optimization, support vectors will have $\gamma_{\rm g, b} = \frac{\beta}{\|w^*_{\rm b}\|_2}$, where $w_b^*$ is the optimal $w_b$. But that's already the best geometric margin we can get for this dataset without violating the $\gamma_{\rm f, b}(x_i, y_i) \geq \beta$ constraint. If we now replace $w_b^*$ by $0.5w^*_b$ (decreasing the norm), for the support vectors, we will have $\gamma_{\rm f, b} = 0.5\beta$ and $\gamma_{\rm g, b} = \frac{\beta}{\|w^*_{\rm b}\|_2}$. So the geometric margin does not change with the norm of $w$ (neither does the classifier). WDYT?}{\color{blue} Ankit: Yes, this post-hoc updating of weights, e.g., $w_{\rm b} \to 0.5 w_{\rm b}$ is not changing geometric margin or the sign of the functional margin. But in the multi-class case below, if we do post-hoc update of the weights for different classes in a different manner, it might change the sign of the 'function' margin $\gamma$ (in \eqref{eq:mc_svm}) for sure.} {\color{red} Agreed! I guess the multi-class equivalent of the above scaling that doesn't affect the geometric margin or the sign of the functional margin would be $W \to 0.5W$, where $W$ is the full weight matrix.

BTW, from http://cs229.stanford.edu/notes/cs229-notes3.pdf it seems that, in the binary case, the intuition behind the geometric margin is that it's a "normalized" functional margin that cannot be changed just by changing the norm of the weights, without changing the final outcome of the classifier after argmax. Now, for the multiclass case we have the functional margin,
$$
\gamma_{\rm f}(x, y) = w_y\cdot\phi(x) - \max_{y' \neq y} w_{y'}\cdot\phi(x).
$$
We can arbitrarily change the above functional margin without changing the final behaviour of the classifier by multiplying the norm of \emph{each} $w_i$ by the same multiplier (e.g. $W \to 0.5W$ case above). This agrees well with the nature of the functional margin in the binary case. Now, wouldn't the geometric margin for the multiclass case be something like
$$
\gamma_{\rm g}(x, y) = \frac{w_y\cdot\phi(x) - \max_{y' \neq y} w_{y'}\cdot\phi(x)}{\|W\|_F},
$$
where $\|W\|_F$ is the Frobenius norm of the whole weight matrix? If we define the geometric margin this way, it cannot be arbitrarily changed without changing the primary behavior of the classifier (this was the motivation for defining the geometric margin for the binary case as well?). Note the difference between the above definition and Eq. (9). Essentially, I'm still unclear that $\|w_y\|$ is a proxy for the geometric margin?
} {\color{blue}Ankit: You are right. We should define $\gamma_{\rm g}(x, y) = \gamma_{\rm f}(x, y)/{\rm norm}(W)$ and then minimize that norm. In \eqref{eq:mc_svm}, we are using ${\rm norm}(W) = \|W\|_{2,1}$, but we can replace it with $\|W\|_F$. My bad. I basically came up with \eqref{eq:g_margin_mc} by looking at \eqref{eq:mc_svm} and \eqref{eq:binary_svm}.}
%

Based on the same logic, we can talk about the `geometric' margin of $(x, y)$ in the multiclass case and define it to be the distance of $(x, y)$ from it's classifier, i.e.,
\begin{align}
\label{eq:g_margin_mc}
\gamma_{\rm g} = \frac{|w_{y}\cdot\phi(x)|}{\|w_{y}\|_2}.
\end{align}
Now again, we can make sure that our classifier classifies $(x, y)$ correctly by ensuring $\gamma(x, y) > 0$ and then further make sure that correctly classified points are as far as possible from their classifier by minimizing $\|w_y\|_2$. This gives us the hard-SVM in the multiclass setting as 
\begin{equation}
\begin{aligned}
\label{eq:mc_svm}
\min_{w} \quad & \sum_{c \in \YCal}\|w_c\|_2 \\
\textrm{s.t.} \quad & \gamma(x_i, y_i) = w_y\cdot\phi(x) - \max_{y' \neq y} w_{y'}\cdot\phi(x) > 0~~\forall i \in [n].\\
\end{aligned}
\end{equation}

\begin{remark}
So, the norms ${\|w_c\|_2}_{c\in \YCal}$ are the correct proxy for the 'geometric' margin even in the multiclass classification. Since we saw in the colab that SGD+momentum is already providing small class norms to the rarer classes, so it might already be ensuring good margin on the rarer class. However, in the multiclass setting, it's a bit tricky. Even though small norm $\|w_y\|_2$ ensures that $(x, y)$ is very far from its classifier, it may also lead to $\gamma(x, y) = w_y\cdot\phi(x) - \max_{y' \neq y} w_{y'}\cdot\phi(x) < 0$. So the question of generalization and small error on training data are a bit entangled.
\end{remark}

